Crowdsourcing Pareto-Optimal Object Finding by Pairwise Comparisons

This is the first study on crowdsourcing Pareto-optimal object finding, which has applications in public opinion collection, group decision making, and information exploration. Departing from prior studies on crowdsourcing skyline and ranking queries, it considers the case where objects do not have explicit attributes and preference relations on objects are strict partial orders. The partial orders are derived by aggregating crowdsourcers' responses to pairwise comparison questions. The goal is to find all Pareto-optimal objects by the fewest possible questions. It employs an iterative question-selection framework. Guided by the principle of eagerly identifying non-Pareto optimal objects, the framework only chooses candidate questions which must satisfy three conditions. This design is both sufficient and efficient, as it is proven to find a short terminal question sequence. The framework is further steered by two ideas---macro-ordering and micro-ordering. By different micro-ordering heuristics, the framework is instantiated into several algorithms with varying power in pruning questions. Experiment results using both real crowdsourcing marketplace and simulations exhibited not only orders of magnitude reductions in questions when compared with a brute-force approach, but also close-to-optimal performance from the most efficient instantiation.

==> sec-problem.tex <==
\section{Concepts}
\subsection{Pareto-optimal Objects}\label{sec:concept}
Consider a set of objects $O$ and a set of criteria $C$ for comparing
the objects.  For each individual criterion $c \in C$, a
\emph{preference relation} $P_c$ (also denoted $\succ_c$) over $O$ is a
binary relation subsumed by $O \times O$, in which $(\obj{x},\obj{y})\in P_c$ (also
denoted \domC{x}{y}{c}) is interpreted as ``\obj{x} is better than (preferred
than) \obj{y} with regard to criterion $c$''.  Hence, if $(\obj{x},\obj{y})\notin P_c$
(also denoted $\obj{x} \nsucc_c \obj{y}$), \obj{x} is not better than \obj{y} by criterion
$c$.  We say \obj{x} and \obj{y} are \emph{indifferent} by criterion $c$ (denoted
\indiffC{x}{y}{c}), if $(\obj{x},\obj{y}) \notin P_c \wedge (\obj{y},\obj{x}) \notin P_c$, i.e.,
``\obj{x} and \obj{y} are equally good or incomparable with regard to criterion
$c$.''  $P_c$ is a \emph{strict partial order}, i.e., $P_c$ is irreflexive
($\forall \obj{x}, (\obj{x},\obj{x}) \notin P_c$) and transitive ($\forall \obj{x},\obj{y}, (\obj{x},\obj{y}) \in
P_c \wedge (\obj{y},\obj{z}) \in P_c \Rightarrow (\obj{x},\obj{z}) \in P_c$), which together also
imply asymmetry ($\forall \obj{x},\obj{y}, (\obj{x},\obj{y}) \in P_c \Rightarrow (\obj{y},\obj{x}) \notin P_c$).
Note that strict partial order was also used in modeling preference
queries~\cite{kiessling2002foundations,chomicki2003preference,chomicki2011logical}
and skyline queries over partially ordered domains~\cite{skylinepartialorder-zhang-vldb10}.

Under the preference relations over a set of criteria $C$, given objects
\obj{x}, \obj{y} $\in O$, \obj{x} dominates \obj{y} (denoted \domO{x}{y}) if and only if
\obj{y} is not better than \obj{x} by any criterion and \obj{x} is better than \obj{y} by
at least one criterion, i.e.,
\begin{center}
$\forall c\in C, \obj{y} \nsucc_c \obj{x}$ and $\exists c\in C$ such that \domC{x}{y}{c}.
\end{center}
If \obj{x} and \obj{y} do not dominate each other (i.e., $\obj{x}\nsucc \obj{y}$ and $\obj{y}
\nsucc \obj{x}$),  we denote it by \indiffO{x}{y}.  \obj{x} is a \emph{Pareto-optimal
object} if and only if \obj{x} is not dominated by any other object, i.e.,
$\nexists \obj{y}\in O$ such that \domO{y}{x}.  This definition of Pareto-optimality
on multiple partial orders was also adopted in~\cite{skylinepartialorder-zhang-vldb10}.

We use Example~\ref{ex:movie} to explain the concepts defined above.  The
objects are $O=\{ \obj{a,b,c,d,e,f} \}$ and the criteria are $C=\{ story,$
$music,$ $acting \}$.  In the ensuing discussion, we denote the three criteria
by $s$, $m$, and $a$, respectively.  An example tuple in a preference
relation is $(\obj{a},\obj{e})$$\in$$P_m$, i.e., \domC{a}{e}{m}.
$(\obj{b},\obj{d})$$\notin$$P_s$ and $(\obj{d},\obj{b})$$\notin$$P_s$, hence \indiffC{b}{d}{s}.
Movie \obj{c} dominates \obj{d}
(\domO{c}{d}), because \obj{c} is preferred than \obj{d} on \emph{story} and
\emph{music} and they are indifferent on \emph{acting}, i.e.,
\domC{c}{d}{s}, \domC{c}{d}{m}, and \indiffC{c}{d}{a}.  Movies \obj{a} and \obj{b} do not dominate each other, i.e., \indiffO{a}{b}, since \domC{b}{a}{s}, \domC{a}{b}{m} and \domC{b}{a}{a}.  Movie \obj{b} is Pareto-optimal since no other movies dominate it.

